Reducing Alert Fatigue via AI-Assisted Negotiation: A Case for Dependabot

The increasing complexity of software dependencies has led to the emergence of automated dependency management tools, such as Dependabot. However, these tools often overwhelm developers with a high volume of alerts and notifications, leading to alert fatigue. This paper presents a position on using Artificial Intelligence (AI) agents as dependency negotiators to reduce alert fatigue. We then examine specific use cases where AI agents can facilitate dependency negotiations, such as when working with external dependencies or managing complex, multi-component systems. Our findings highlight the need for more research on the design and evaluation of AI-driven dependency mediation mechanisms. With a focus on ensuring transparency, explainability, and human trustworthiness in these GitHub software projects, our goal is to reduce alert fatigue to an extent that maintainers no longer feel overwhelmed and welcome pull requests just like any other contribution into their projects.

==> sections/1_introduction.tex <==
\section{Introduction}
\label{1_introduction}

Open-source software has become a fundamental component of technological advancement and is used by individuals and organizations worldwide. This impact is especially evident in fields like data science, where open-source tools provide foundational support and enable complex analyses that would be challenging without community-driven resources. \cite{Malone2020Doing}
% \morakot{cite}
This reusable code is publicly available in online repositories and delivered by software management systems, such as npm for Node.js or Python Package Index (PyPI)\cite{PyPI} for Python packages. These repositories host an extensive collection of reusable code, offering numerous benefits by providing reusable code to save time and effort in software development, these libraries are widely reused among developers. 
\cite{DBLP:journals/corr/abs-1907-11073}
% \morakot{cite}
With this widespread usage comes a dependence on packages, increasing the spread of vulnerability problems through reused packages.

Existing research underscores the critical role of security policies in effectively managing vulnerabilities within open-source software. Nusrat Zahan et al. \cite{zahan2023softwaresecuritypracticesyield} recommend for a comprehensive approach to security practices, including the implementation of security policies that incorporate best practices in project management and secure development. This viewpoint highlights the necessity of a proactive and holistic strategy for security, aimed at addressing vulnerabilities throughout the software development lifecycle.
ecurity, addressing vulnerabilities throughout the software lifecycle.
Ayala, Garcia, et al. \cite{10190609} conducted an empirical study of GitHub workflows and security policies in popular repositories, finding that only 37\% of repositories have workflows enabled, and only 7\% have defined security policies. The study also highlights limited adoption of CodeQL, GitHub's static analysis tool for vulnerability detection, with only 13.5\% of applicable repositories utilizing it. Zahan et al. \cite{10163720} analyze security practices in npm and PyPI using the OpenSSF Scorecard, which assesses projects based on security metrics such as workflow configuration and vulnerability reporting. Their study reveals notable security gaps and low adoption rates of best practices, finding that security policies recommended by GitHub are implemented in fewer than 4\% of projects. 
These findings emphasize the need for open-source project maintainers to prioritize workflow configuration, automated static analysis, and security policy definition to mitigate vulnerabilities and strengthen the security of widely-used software in the supply chain. Additionally, they underscore the importance of consistent security measures, suggesting that adopting standardized security policies could significantly improve open-source security.
The security of the software packages is the backbone of numerous applications used in the industry. It is essential to ensure that these packages maintain a security posture because they are publicly accessible and unaddressed vulnerabilities can have significant consequences for their users. Fixing the vulnerabilities rapidly after their discovery is essential, especially after the vulnerabilities have been publicly disclosed. Alfadel et al. \cite{EmpiricalAnalysisOfSecurityVulnerabilitiesInPythonPackages} analyzed the security vulnerability in PyPI for Python packages, and found that the vulnerability in PyPI packages has been increasing over time, with some projects taking a long time to disclose and fix the vulnerabilities.

\begin{figure*}[ht!] 
    \centering
    \includegraphics[width=0.8\linewidth, 
    % height= 0.19\linewidth
    ]
    {3RQsFlowFinal_Fixed.png}
    \caption{Overview of the study}
    \label{fig:overviewFig}
\end{figure*}

Given the critical need for maintaining security in open-source software, platforms hosting these repositories have a role in supporting security practices. GitHub, one of the largest platforms for open-source code, provides maintainers with tools to establish and communicate security guidelines directly within the project repository. This includes the ability to add a SECURITY.md file \cite{GitMd}, a dedicated document for outlining the project's vulnerability disclosure process, reporting steps, and security-related guidelines. By offering this feature, GitHub encourages maintainers to adopt a proactive approach to managing security, helping developers address vulnerabilities efficiently and transparently. A study by Ayala and Garcia~\cite{10190609} suggests that maintainers should prioritize adding a security policy to their projects, as this can help prevent vulnerabilities from lingering in the source code. While GitHub's guidelines emphasize the importance of a reporting mechanism through tools like SECURITY.md, Nusrat et al.~\cite{zahan2023softwaresecuritypracticesyield} suggest that security practices including security policy should cover a broader scope, covering all aspects of best practices in project management and secure software development. This holistic approach can better support maintainers in proactively managing vulnerabilities. 




Our study builds on this premise by investigating the specific contents and structures that constitute effective security policies. By identifying patterns within these policies, we aim to provide open-source pracitioners (e.g., maintainers) with insights that can optimize security management and reduce project vulnerabilities. Despite the crucial role of security policies in managing vulnerabilities, there is limited research study focused on the characteristics of these policies. The primary goal of our study is to identify patterns in defining effective security policies, which can serve as a valuable reference for open-source maintainers. This paper conducts a preliminary investigation into the characteristics, content, and structures that define security policies in software repositories. We first examine the main categories of security policies, identify common patterns within them, and analyze how these policies correlate with specific repository characteristics. By addressing these aspects, this study aims to provide a foundation for developing strategies that enhance security management practices in software development environments. We thus define three research questions to guide our study as follows:


\begin{enumerate}
\item RQ1: What are the primary categories of security policies commonly declared in software repositories?

% \item RQ2: Are there any correlations or associations among the categories of security policies in software repositories?

\item RQ2: Do security policies follow the GitHub template?

\item RQ3: Does the occurrence of security policy categories correlate with characteristics of software repositories?
\end{enumerate}

Our preliminary study of over 300 security policies in open-source projects reveals nine distinct categories of security policy content. Most security policies include a reporting mechanism but rarely outline the procedural steps that will be followed once a vulnerability is reported. Analysis of the co-occurrence of these categories also indicates that user guidelines, such as instructions for secure dependency usage, recommended configurations, and general project usage, are more commonly present in projects that incorporate all basic categories recommended by GitHub. The remainder of this paper provides an in-depth discussion of our study's methodology, findings, and implications.


% Thus, this paper aims to investigate the contents and structures that constitute well-defined security policies, finding how these can be optimized for better security management.
% \morakot{says something about the big goal of the study. the big goal is that we want to find a good pattern in definding security policy} \morakot{says that thus this paper aim to initially investigate ....}

% This gap in the literature, especially regarding the content and structure of security policies, motivates our investigation into their defining characteristics.\chaiyong{I think this repeats the previous paragraph. Need paraphrasing or removal.}

% We define three research questions to guide our preliminary study:

% \morakot{We define three resaerch questions to guild our preliminary study as follows:}

% \begin{enumerate}
% \item \textbf{RQ1:} What are the main categories of security policies in software repositories?

% \item \textbf{RQ2:} What common patterns can be observed within security policies across repositories?

% \item \textbf{RQ3:} How do security policies correlate with specific repository characteristics?
% \end{enumerate}

% \morakot{RQ1: What are the main categories of security policies in software repositories?
% RQ2: What common patterns can be observed within security policies across repositories?
% RQ3: How do security policies correlate with specific repository characteristics?}



%  \morakot{says briefly about our finding}

% \morakot{We thus conducted the student on xxxx Github repositoies with secrueirty.md. We found that ......}

% To address these research questions, we analyzed 303 security policies within 679 PyPI projects found in GitHub’s advisories report. Our study categorizes security policy contents into nine distinct categories and examines the frequency and context of these categories to identify those most commonly utilized across projects. Through this analysis, we aim to provide insights that can help maintainers enhance the security readiness of their repositories by establishing clear, structured, and comprehensive security guidelines.

% \morakot{The rest of this paper is organized as follows. Section II provides existent studies on commit message generation and applications of LLMs. Section III presents the research questions of this work and the overview of our approach. Section IV is the results and discussion.}

==> sections/2_background.tex <==
\section{GitHub Security Policy}



\label{2_background}

% In this section, we review prior research on GitHub’s security policy feature and its role in open-source software, focusing on key findings regarding its impact on vulnerability handling and community trust. We also identify gaps in the current literature related to security policy adoption and effectiveness in open-source projects.


% \subsection{GitHub Security Policy}
GitHub introduced the security policy feature to help projects formalize their approach to vulnerability handling. This policy is typically provided as a SECURITY.md file, located either in the project’s main directory or the .github directory. This file guides users and contributors on reporting security vulnerabilities and outlines any established guidelines for handling these issues. In an official blog post from May 2019, GitHub highlighted the role of the SECURITY.md file in specifying a repository's security policy. When included, this file appears in the repository’s \textit{Security} tab and within the new issue workflow, facilitating more accessible reporting procedures for contributors \cite{githubSecurityPolicy2019}. In November 2022, GitHub emphasized the significance of the SECURITY.md file by further highlighting the security policy on the repository overview in the sidebar. This adjustment further emphasizes its accessibility to users and contributors \cite{githubSecurityPolicy2022}. According to GitHub’s documentation,\footnote{\url{https://docs.github.com/en/code-security/getting-started/adding-a-security-policy-to-your-repository}
} a clear security policy can improve responsiveness to security reports, assist maintainers in prioritizing critical issues, and foster trust. GitHub also offers a security policy template to help maintainers create their policies. 

% \chaiyong{Do we know since when? We may need a citation here.}
% \pooh{I had found the blog post.}

% \pooh{because its quite recent? (is 2 years recent?) should I emphasize how recent the precise it is?}




% Figure \ref{figure:template} shows the template includes three sections: \textit{Security Policy}, \textit{Supported Versions} (listing versions currently maintained with security updates), and \textit{Reporting a Vulnerability}, which specifies the procedure for reporting security issues.
% {

% \begin{figure}

%     \centering
% \begin{mdframed}[linewidth=1pt, roundcorner=10pt]

% \# Security Policy

% \#\# Supported Versions

% Use this section to tell people about which versions of your project are
% currently being supported with security updates.
% \vspace{10pt}

% \begin{tabular}{|l|c|}
% \hline
% \textbf{Version} & \textbf{Supported} \\
% \hline
% 5.1.x & \checkmark \\
% 5.0.x & \texttimes \\
% 4.0.x & \checkmark \\
% \textless{} 4.0 & \texttimes \\
% \hline
% \end{tabular}

% \vspace{10pt}
% \#\# Reporting a Vulnerability

% Use this section to tell people how to report a vulnerability.

% Tell them where to go, how often they can expect to get an update on a
% reported vulnerability, what to expect if the vulnerability is accepted or
% declined, etc.
% \end{mdframed}
% \caption{Security Policy Template provided by GitHub}
% \label{figure:template}
% \end{figure}

% % \morakot{add footnote as a url to the page of github template guidline}
% % \pooh{the template guideline can be access via a security tab inside a project, therefor you need a repository to view it. to compensate, I insert a fig1 for the template with a footnote to documentation instead.}

% % \morakot{add example of sec.md}

% \subsection{Related works}

% Existing research underscores the critical role of security policies in effectively managing vulnerabilities within open-source software. Nusrat Zahan et al. \cite{zahan2023softwaresecuritypracticesyield} recommend for a comprehensive approach to security practices, including the implementation of security policies that incorporate best practices in project management and secure development. This viewpoint highlights the necessity of a proactive and holistic strategy for security, aimed at addressing vulnerabilities throughout the software development lifecycle.


% % Most related work explores the importance of security policies in managing vulnerabilities within open-source software. Nusrat Zahan et al. \cite{zahan2023softwaresecuritypracticesyield} suggest that security practices, including security policies, should adopt a comprehensive approach that encompasses best practices in project management and secure development. This perspective emphasizes the need for a more proactive and holistic approach to security, addressing vulnerabilities throughout the software lifecycle.

% Ayala, Garcia, et al. \cite{10190609} conducted an empirical study of GitHub workflows and security policies in popular repositories, finding that only 37\% of repositories have workflows enabled, and only 7\% have defined security policies. The study also highlights limited adoption of CodeQL, GitHub's static analysis tool for vulnerability detection, with only 13.5\% of applicable repositories utilizing it. Zahan et al. \cite{10163720} analyze security practices in npm and PyPI using the OpenSSF Scorecard, which assesses projects based on security metrics such as workflow configuration and vulnerability reporting. Their study reveals notable security gaps and low adoption rates of best practices, finding that security policies recommended by GitHub are implemented in fewer than 4\% of projects. 


% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.5\linewidth]{3RQsFlowFinal.png}
% %     \caption{Enter Caption}
% %     \label{fig:enter-label}
% % \end{figure}



% These findings emphasize the need for open-source project maintainers to prioritize workflow configuration, automated static analysis, and security policy definition to mitigate vulnerabilities and strengthen the security of widely-used software in the supply chain. Additionally, they underscore the importance of consistent security measures, suggesting that adopting standardized security policies could significantly improve open-source security. Our work aims to address these gaps by proposing solutions that enhance security practices and support maintainers in implementing effective, standardized policies across open-source projects.

% \morakot{missing}

==> sections/3_methodology.tex <==
\section{Methodology}
\label{3_methodology}
\usetikzlibrary{shapes, arrows.meta, positioning}
In this section, we present the methodology



\subsection{Overview} 
Figure \ref{fig:overviewFig} shows an overview of our study framework. The study begins with the collection of vulnerability report data from GitHub Advisory, specifically focusing on PyPI packages. While this initial scope centers on PyPI, future work will aim to broaden the range of analyzed packages. From the vulnerability reports, we extract a list of relevant PyPI projects and gather the corresponding GitHub repositories for further analysis. Once the repositories are collected, we identify those containing a security policy file (e.g., SECURITY.md), which serves as the primary data source for our study. Following data collection, we preprocess the repositories to extract relevant content from the security policies, such as policy categories and specific features characterizing each repository. This refined dataset enables us to address our research questions. For RQ1, we manually examine and categorize the security policy content. For RQ2, we apply association rule mining\cite{ReadME}
% \morakot{cite}\pooh{cited} 
to analyze patterns within the dataset. For RQ3, we conduct a correlation analysis to explore the relationship between project characteristics and identified security policy categories. A detailed description of our study’s methodology follows.

% , gathering a total of 2,311 reports on PyPI packages. We can then retreive the list of 679 unique PyPI projects existing in GitHub Advisory. We can then identify 



% \morakot{some of these details we can move to their subsection e.g. the number reporting. the overview should be just describe the methodology in general}
% Our study methodology is outlined in \ref{fig:enter-label}, illustrating the process of analyzing security policies across PyPI projects. We begin with data collection from GitHub Advisory, gathering a total of 2,311 reports on PyPI packages. Through data preprocessing, these reports are filtered to identify 679 unique PyPI packages, of which 303 contain an explicit security policy. From these policies, we extract a total of 722 content blocks, which represent distinct sections of security-relevant information. To categorize and understand the themes within these policies, we employ content snowballing and manual analysis, aiming to answer our first research question (RQ1) by identifying the primary security policy categories. Additionally, we use association rule mining to detect common patterns and relationships among these categories, addressing our second research question (RQ2) on frequently occurring security policy themes. Finally, collocation analysis is applied to examine the spatial relationships and co-occurrence of security policy elements within project features, helping us answer our third research question (RQ3) on how security policies are positioned in relation to project components. This multi-step approach allows us to uncover and characterize patterns in the content and structure of security policies across open-source projects.

% \morakot{need framework figure}

% - figure overview framework





% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{2RqFlow.png}
%     \caption{Framework Overview}
%     \label{fig:enter-label}
% \end{figure}

% \morakot{use section command}
\subsection{Data Collection} 

Our study examines the security policies of open-source projects within the PyPI ecosystem, specifically focusing on projects listed in GitHub’s advisory database. Data collection begins with querying the GitHub Advisory API\footnote{\url{https://docs.github.com/en/graphql/reference/queries\#securityadvisories}}
% \morakot{add footnote to the API manual}\pooh{added}
to retrieve a total of 2,311 advisory reports on PyPI packages. From this data, we extract a list of unique PyPI projects, accounting for instances where multiple reports pertain to a single project. This refinement results in 679 unique projects.
A security policy file in a repository can be implemented in various ways, including placement within the project repository or within the \texttt{.github} repository. It can be located in directories such as the project root, the \texttt{.github} folder, or the \texttt{docs} folder. The security policy file can be labeled as ``security'' (case-insensitive) and may exist in \texttt{.md} or \texttt{.rst} formats. During data preprocessing, we filter the reports to identify these unique PyPI packages, of which 303 contain a clear security policy. We then proceed to gather the corresponding GitHub repositories for further analysis.



% //Pooh, I know that "including, but not limited to" is not academic but I want to show the possible location of policy. cause as far as I know, I could not find any site mentioning this. and importantly I could not proof that this is all the possible locations it ban be.

% \vspace{10pt}

% \begin{figure}[h!]
% \centering
% \begin{tikzpicture}[node distance=2cm, font=\small]
% % Nodes
% \node (start) [startstop] {Start};
% \node (repo) [decision, below of=start, yshift=0.25cm] {Repository};
% \node (projRepo) [process, below of=repo, xshift=-1.5cm, yshift=0.5cm] {Project Repository};
% \node (dotGithubRepo) [process, below of=repo, xshift=1.5cm, yshift=0.5cm] {.github Repository};

% \node (filepath) [decision, below of=repo, yshift=-1cm] {Directory};

% \node (githubDir) [process, below of=filepath, yshift=.35cm] {/.github};
% \node (rootDir) [process, left of=githubDir, xshift=-.5cm] {/\textit{root}};
% \node (docsDir) [process, right of=githubDir, xshift=.5cm] {/docs};

% \node (filename) [decision, below of=githubDir, yshift=.25cm] {File Type};

% \node (securityMd) [process, below of=filename, yshift=.5cm ,xshift=-1.5cm] {.md};

% \node (securityRst) [process, below of=filename, yshift=.5cm ,xshift=1.5cm] {.rst};

% % Arrows
% \draw [arrow] (start) -- (repo);
% \draw [arrow] (repo) --  (projRepo);
% \draw [arrow] (repo) -- (dotGithubRepo);

% \draw [arrow] (projRepo) -- (filepath);
% \draw [arrow] (dotGithubRepo) -- (filepath);

% \draw [arrow] (filepath) -- (rootDir);
% \draw [arrow] (filepath) -- (githubDir);
% \draw [arrow] (filepath) -- (docsDir);

% \draw [arrow] (rootDir) -- (filename);
% \draw [arrow] (githubDir) -- (filename);
% \draw [arrow] (docsDir) -- (filename);

% \draw [arrow] (filename) -- (securityMd);
% \draw [arrow] (filename) -- (securityRst);

% \end{tikzpicture}
% \caption{Possibility of Security Policy Source File\chaiyong{Not sure we need this figure. If we need to save space, this may go.}}
% \label{fig:security-policy}
% \end{figure}






% https://www.tablesgenerator.com/

% \begin{table}[tb]
% \centering
% \begin{tabular}{lll|r|l}
% \cline{1-4}
% \multicolumn{3}{c|}{Extraction Snapshot of Reports} & \multicolumn{1}{c|}{Oct 2024} &  \\ \cline{1-4}
% \multicolumn{3}{l|}{PyPI Report from GitHub's Advisory} & 2311 reports &  \\ \cline{2-4}
% \multicolumn{1}{l|}{} & \multicolumn{2}{l|}{Unique PyPI Project from GitHub's Advisory} & 679 Projects &  \\ \cline{3-4}
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & PyPI projects with security policy & 303 Projects   &  \\ \cline{1-4}
% \end{tabular}
% \vspace{10pt}
% \caption{Summary of Extracted PyPI projects.\chaiyong{Strange table format. I think this is better represented using a figure showing the filtering of the data from left $\rightarrow$ right.}}
% \label{tab:pypi_data_tables}
% \end{table}


\subsection{Data Preprocessing} 


After acquiring the security policies from unique PyPI projects listed in GitHub's Advisory reports, we parsed the titles and content based on markdown formatting. Specifically, we identified each security policy \texttt{content block} as starting with a title marked by a hashtag symbol (\#) followed by its associated content. This approach allowed us to build datasets containing the security policy content blocks within the PyPI ecosystem. Figure \ref{fig:data_filtering} shows the data filtering process, where each content block is extracted, cleaned, and structured for further analysis. From these policies, we extract a total of 722 content blocks, which represent distinct sections of security-relevant information. 


\begin{figure}[H]
    \centering
    \begin{tikzpicture}[
        block/.style={
            rectangle, draw, thin, minimum height=2.5cm, minimum width=1cm, anchor = base,
            align=center, font=\small, fill=gray!10
        },
    ]

    % Blocks with captions and numbers
    \node[block] (stage1) {PyPI\\Vulnerability\\Reports from \\GitHub\\Advisory\\\rule{1.5cm}{0.4pt}\\2311 reports\\};
    
    \node[block, right=of stage1, xshift=-.65cm] (stage2) {Unique PyPI\\Projects with\\Vulnerability\\Reports\\\\\rule{1.5cm}{0.4pt}\\679 Projects\\};
    
    \node[block, right=of stage2, xshift=-.65cm] (stage3) {PyPI Projects\\Containing\\Security\\Policies\\\\\rule{1.5cm}{0.4pt}\\303 Projects\\};
    
    \node[block, right=of stage3, xshift=-.65cm] (stage4) { Extracted\\Security \\Policy\\Content\\ Blocks\\\ \rule{1.5cm}{0.4pt}\\722 Content \\Blocks};

    % Arrows
    \draw[arrow] (stage1) -- (stage2);
    \draw[arrow] (stage2) -- (stage3);
    \draw[arrow] (stage3) -- (stage4);

    \end{tikzpicture}
    \caption{Summary of data collection and preprocessing steps}
    \label{fig:data_filtering}
    
\end{figure}


% The projects without security policies are ruled out. We obtained 303 unique PyPI projects with security policy.
% \vspace{10pt}

% \begin{table}[h!]
% \centering
% \begin{tabular}{llll|r|l}
% \cline{1-5}
% \multicolumn{4}{c|}{Extraction Snapshot of Reports} & \multicolumn{1}{c|}{Oct 2024} &  \\ \cline{1-5}
% \multicolumn{4}{l|}{PyPI Report from GitHub's Advisory} & 2311 Reports &  \\ \cline{2-5}
% \multicolumn{1}{l|}{} & \multicolumn{3}{l|}{Unique PyPI Project from GitHub's Advisory} & 679 Projects &  \\ \cline{3-5}
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{2}{l|}{Unique PyPI projects with security policy} & 303 Projects &  \\ \cline{4-5}
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \textbf{PyPI Security Policy content block} & \multicolumn{1}{l|}{\textbf{722 Content Blocks}} &  \\ \cline{1-5}
% \end{tabular}
% \vspace{10pt}
% \caption{Summary of Extracted PyPI Content Blocks.\chaiyong{Similar to the Table I.}}
% \label{tab:pypi_data_tables_2}
% \end{table}


\subsection{Data Analysis} 

\subsubsection{RQ1: What are the primary categories of security policies commonly declared in software repositories?}

To address RQ1, we conducted a manual analysis using Cohen's Kappa \cite{Cohen} 
% \morakot{cite cohen kappa original paper}\pooh{cited}
to ensure reliability. Our process involved an iterative approach, where we examined documents one by one, refining and expanding categories as each new document was analyzed. This iterative method allowed for a comprehensive and detailed set of categories to emerge naturally from the data. For each security policy content block, two researchers independently categorized the content without prior knowledge of each other's categorization choices. Following the initial categorization, we calculated Cohen's Kappa to assess the reliability of the manual analysis, ensuring consistency and minimizing the influence of individual biases. 

In cases where disagreements occurred, the assigned pair engaged in a discussion session to review and resolve conflicts, reaching a consensus on the final categorization. This collaborative resolution process reinforced the reliability of the categorized content blocks. After finalizing the categorizations, we calculated the frequency of each category to identify the most commonly declared security policy types in software repositories. 


% To answer the RQ1, we used a Manual Analysis analysis with Cohen’s Kappa,  \morakot{cite the cohen kappa paper}. We perform an iterative process used to identify categories by reviewing documents one at a time, refining and expanding categories as each new document is analyzed. This allows for a comprehensive set of themes to emerge naturally from the data.

% Manual Analysis with Multiple Investigators: For each security policy content block, a pair of researchers were assigned to independently categorize the content, with no prior knowledge of the other’s categorization choices. After initial categorization, we calculated Cohen’s Kappa to assess manual analysis reliability, ensuring the categorization was consistent and not influenced by individual biases.

% For content blocks where disagreements happen, the assigned pair conducted a discussion session to review and resolve these conflicts, reaching a consensus on the final categorization. This collaborative resolution process strengthened the reliability of the categorized content block.

% We can then determine the frequency count of the appearing of each categories to identify categories of security policies that mostly declared. 


% \chaiyong{inter-rater agreement is not an approach. The actual approach is manual analysis with multiple investigators.}
% \chaiyong{I think this can be removed. You need to explain instead how the two investigators work. Do they look at the policy independently? Do they meet to resolve the conflicts at the end? etc.} \pooh{resolved}

\subsubsection{RQ2: Do security policies follow the GitHub template?}

To address RQ2, we applied association rule mining to identify common patterns within security policies across repositories \cite{AssociationRuleMiningBook, ReadME}. Association rule mining is a data-mining technique that uncovers patterns of co-occurrence among categories in a dataset. By applying this method, we can detect commonly grouped elements, revealing structural similarities across security policies in different repositories.

In our analysis, we used the support metric to measure the significance of these patterns. The support metric indicates the proportion of repositories in the dataset where a specific combination of categories is present. To calculate the percentage of repositories adhering to GitHub's recommended security policy template, we identified itemsets that included the category found within GitHub's security policy template. The support value for this itemset was then multiplied by 100 to express the adherence rate as a percentage. Similarly, the percentage of repositories not adhering to the template was computed as 100 Adherence Percentage

This approach allows us to quantitatively assess the extent to which repositories follow GitHub's template and identify additional patterns or extensions commonly included by maintainers.


% This approach provides insight into the common structures and priorities in security policies within the PyPI ecosystem.

% To address RQ2, we applied association rule mining to identify common patterns within security policies across repositories \cite{AssociationRuleMiningBook, ReadME}. Association Rule Mining is a data-mining technique used to identify patterns of co-occurrence among categories in a dataset. Applying metrics like support frequently reveals co-existing elements, highlighting common structures across items in the data. [explain in our context as well]

% To measure the significance of these patterns, we used the support metric, which indicates how frequently certain category combinations occur across the dataset. High-support patterns reveal commonly co-existing elements in security policies, helping us identify the foundational components that are widely shared in open-source repositories.
\begin{table*}[!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{3.5cm}rp{5cm}p{8.5cm}}
\toprule
\textbf{Category} & \textbf{Count} & \textbf{Definition} & \textbf{Example} \\
\midrule
\textbf{Reporting mechanism} & 282 & A set of instructions outlining the procedure for reporting security vulnerabilities to the relevant developers. & {``To report a vulnerability, please do not share it publicly on GitHub nor the community slack channel. Instead, contact the \censortext \ \ team directly via email first: \censortext \ ''} \\

\textbf{Generic policy} & 211 & Outline objective and foundation of security policy. & ``This document describes model security and code security in \censortext. It also provides guidelines on how to report vulnerabilities in \censortext.'' \\

\textbf{User guideline} & 133 & Security-related and project-specific e.g. Instructions for users, including secure usage of dependencies, recommended configurations, and general project usage. & ``\censortext \ \ is not intended to be deployed on a public-facing server. By default, the web UI is only exposed on localhost, so normally this is not a problem. Do not give someone access to the web UI unless you trust them with everything else that is on that machine.'' \\

\textbf{Scope of practice} & 127 &The list of project versions still under maintenance. & ``These \censortext \ \ releases are currently supported with security updates: Version 1.2.x - \checkmark\  Supported Version \textless{}1.1 - \texttimes\ Not supported'' \\

\textbf{Project practice} & 20 & Detailed procedural steps that will be executed when a vulnerability is reported. & ``Each report is acknowledged and analyzed by security response members within five (5) working days. Any vulnerability information shared with security response members stays within the \censortext \ \ project and will not be disseminated to other projects unless it is necessary to get the issue fixed.'' \\

\textbf{History of vulnerability} & 8 & A list of disclosed vulnerabilities. & ``We maintain Security Advisories on the \censortext \ \ project \censortext \ \ repository, where we will post a summary, remediation, and mitigation details for any patch containing security fixes." \\

\textbf{Additional information} & 7 & Non-security related and project specific e.g. Access for further details that are non-related to the security, Copyright section, project contribution, acknowledgment. & ``We prefer all communications to be in English'' \\

\textbf{Information on maintainer} & 4 & Maintainer information e.g. name, email, role, responsibility. & ``\censortext \ \ is always open to feedback, questions, and suggestions. If you would like to talk to us, please feel free to email us at \censortext \ \, and our PGP key is at \censortext \ .'' \\

\textbf{Others} & 0 & None of all above. & - \\

\bottomrule
\end{tabular}
}
\caption{Categories of Security Policy Titles}
\label{Categories of Security Policy Titles}
\end{table*}


\subsubsection{RQ3: Does the occurrence of security policy categories correlate with characteristics of software repositories?}

In this study, we categorize repositories based on a set of traditional attributes, with plans to expand this feature set in future research. The initial features include project age (in days), number of commits, number of contributors, number of subscribers, number of pull requests, total number of issues, number of open issues, repository size (in kilobytes), number of stars, and number of forks. We then apply point-biserial correlation analysis \cite{Point‐biserial} to examine the correlation between project features and security policy categories. This method is appropriate for identifying correlations between continuous variables (e.g., project features) and binary indicators representing the presence of specific categories. Thus, we can observe which project characteristics are most strongly associated with certain security policy categories.
% For instance, projects with a higher number of contributors or commits may be more likely to implement comprehensive security policies. 


% To explore how security policies correlate \cite{Point‐biserial} with specific repository characteristics, we conducted a point-biserial correlation analysis between project features and security policy categories.

% This approach show the strength and direction of relationships between continuous project features and binary security policy categories. By identifying significant correlations, we aim to reveal which repository characteristics are associated with the presence of specific security policy elements.
% \textbf{Overview of Git Version Control Data}
% \ani{xxx}

==> sections/4_results.tex <==
\section{Results}
\label{4_results}


\subsection{RQ1: What are the primary categories of security policies commonly declared in software repositories?}

% \begin{table}[h]
% \centering
% \begin{tabular}{lp{4.75cm}}
% \toprule
% \textbf{Category} & \textbf{Definition} \\
% \midrule
% \textbf{Generic policy} & Outline objective and foundation of security policy. \\
% \textbf{Reporting mechanism} & A set of instructions outlining the procedure for reporting security vulnerabilities to the relevant developers. \\
% \textbf{Information on maintainer} & Maintainer information e.g. name, email, role, responsibility. \\
% \textbf{Scope of practice} & The list of project versions still under maintenance. \\
% \textbf{Project practice} & Detailed procedural steps that will be executed when a vulnerability is reported. \\
% \textbf{History of vulnerability} & A list of disclosed vulnerabilities. \\
% \textbf{User guideline} & Security related and project specific e.g. Instructions for users, including secure usage of dependencies, recommended configurations, and general project usage. \\
% \textbf{Additional information} & Non-security related and project specific e.g. Access for further details that are non-related to the security, Copyright section, project contribution, acknowledgement. \\
% \textbf{Others} & None of all above. \\
% \bottomrule
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Categories of Security Policy Titles \\(addressing RQ1)}
% \label{Categories}
% \end{table}



From the manual validation of security policy content blocks, we can identify nine distinct categories of security policies. The Cohen’s Kappa value was 0.9, indicating almost perfect agreement among the researchers. Table \ref{Categories of Security Policy Titles} presents definitions for each category and the counts of each identified category.

The \texttt{Reporting mechanism} category has the highest count (282), highlighting its importance across projects. This suggests that a large number of repositories prioritize clear instructions for reporting vulnerabilities, emphasizing communication channels that allow users to report security issues effectively. This aligns with best practices, as reporting mechanisms are essential for timely vulnerability disclosure and management. The \texttt{User guideline} category, appearing 133 times, also shows a strong presence, suggesting that many projects provide users with specific security instructions. This may include advice on secure configurations or recommendations to avoid common security pitfalls, reflecting the maintainers’ focus on enhancing the overall security posture of their software.

In contrast, categories like \texttt{Project practice} (20), \texttt{History of vulnerability} (8), \texttt{Additional information} (7), and \texttt{Information on maintainer} (4) appear far less frequently. The low counts suggest that specific project practices, past vulnerability history, and additional details about maintainers are not commonly documented within formal security policies. This raises the concern that these categories may not be receiving adequate attention in current security policies, potentially overlooking elements that could enhance overall security practices. It prompts us to consider whether these categories should be leveraged more effectively to provide a comprehensive view of security practices.

% \begin{table}[h]
% \centering
% \begin{tabular}{lr}
% \toprule
% \textbf{Category} & \textbf{Count} \\
% \midrule
% \textbf{Reporting mechanism} & 282 \\
% \textbf{Generic policy} & 211 \\
% \textbf{User guideline} & 133 \\
% \textbf{Scope of practice} & 127 \\
% \textbf{Project practice} & 20 \\
% \textbf{History of vulnerability} & 8 \\
% \textbf{Additional information} & 7 \\
% \textbf{Information on maintainer} & 4 \\
% \textbf{Others} & 0 \\
% \midrule
% \textbf{Total} & 722 \\
% \bottomrule
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Distribution of Security Policy Categories in PyPI Population (addressing RQ1)}

% \label{tab:pypi_category_distribution}
% \end{table}

\begin{tcolorbox}[] \textbf{RQ1 Summary}:
Nine security policy categories were identified, with \texttt{Reporting mechanism} (282), \texttt{Generic policy} (211), \texttt{User guideline} (133), and \texttt{Scope of practice} (127) being the most common, highlighting their critical roles.
\end{tcolorbox}

% The findings reveal that "Reporting mechanism," "Generic policy," and "Scope of practice" are the most prevalent categories, with counts of 282, 211, and 127, respectively. This prevalence suggests that a significant number of projects prioritize providing structured instructions for reporting vulnerabilities, establishing general security guidelines, and specifying the versions supported with ongoing maintenance. Together, these categories indicate that many maintainers are following the GitHub Security template, which emphasizes clear communication channels, general security principles, and versioning practices to help users manage security-related concerns effectively. In contrast, categories such as "Project practice" and "History of vulnerability" appear less frequently Further, "Additional information" and "Information on maintainer" are rarely documented, . This rarity implies that non-security-specific details or maintainer contact information may be deemed less critical or might be documented outside of formal security policies.







% To address the main categories of security policies in software repositories, we identified nine distinct categories based on the content within each policy document. Table \ref{tab:security_policy_categories} provides definitions for each category, while Table \ref{tab:pypi_category_distributionsensor} outlines their distribution and includes representative examples.

% The findings reveal that "Reporting mechanism," "Generic policy," and "Scope of practice" are the most prevalent categories, with counts of 282, 211, and 127, respectively. This prevalence suggests that a significant number of projects prioritize providing structured instructions for reporting vulnerabilities, establishing general security guidelines, and specifying the versions supported with ongoing maintenance. Together, these categories indicate that many maintainers are following the GitHub Security template, which emphasizes clear communication channels, general security principles, and versioning practices to help users manage security-related concerns effectively.

% In contrast, categories such as "Project practice" and "History of vulnerability" appear less frequently, with only 20 and 8 occurrences respectively, suggesting that fewer projects have formalized procedural steps for handling vulnerabilities or maintain a public record of past security issues. This lower prevalence may imply that, while vulnerability reporting is prioritized, there is limited visibility into internal practices and historical security documentation.

% Further, "Additional information" and "Information on maintainer" are rarely documented, with only 7 and 4 occurrences, respectively. This rarity implies that non-security-specific details or maintainer contact information may be deemed less critical or might be documented outside of formal security policies. Notably, the "Others" category had no occurrences, suggesting that the categories defined in this study comprehensively cover the types of content found within security policies, validating the applicability of our categorization framework for open-source security policy documentation.

% Overall, while most projects emphasize reporting mechanisms, general security guidelines, and versioning practices, there appears to be less focus on transparency regarding internal procedural practices and historical vulnerability records. These findings provide insight into common categories across open-source repositories and highlight areas where security policies could be expanded to enhance transparency and user guidance.




% \morakot{this content of the investigation approach should be moved to the data analysis approach according to Aj.Aun's comment}\pooh{rewrote this part(Q1)}
% \morakot{discuss the finding a bit e.g., what is the majority of content, what are the common content, what is the least or smallest group of content}



% \subsection{RQ2: Are there any correlations or associations among the categories of security policies in software repositories?}

%  The results of our association rule mining show in Figure \ref{fig:PyPIARM_FixedSize}. There are four categories exhibit strong support and frequently co-occur within security policies: \texttt{Generic Policy}, \texttt{Reporting Mechanism}, \texttt{Scope of Practice}, and \texttt{User Guideline}. Notably, these categories align with GitHub's security policy template, which is recommended by GitHub

% However, the \texttt{User Guideline} category does not appear in GitHub's template, yet our analysis shows that maintainers frequently include it alongside GitHub's recommended categories. This suggests that maintainers see value in providing specific security instructions for users, considering it an important addition to core policy elements and a way to enhance security practices across repositories.



\subsection{RQ2: Do security policies follow the GitHub template?}

The results of our association rule mining, reveal that 39.93\% of repositories adhere to GitHub's recommended security policy template by including all three core categories: \texttt{Generic Policy}, \texttt{Reporting Mechanism}, and \texttt{Scope of Practice}. However, the remaining 60.07\% of repositories either omit one or more of these categories or incorporate additional elements, indicating that not all maintainers strictly follow the template.

Interestingly, our analysis highlights the frequent inclusion of the \texttt{User Guideline} category, which is absent from GitHub's template but co-occurs frequently alongside the recommended categories. This suggests that maintainers see value in providing specific security instructions for users, considering it an important enhancement to the core policy elements is shown in Figure \ref{fig:PyPIARM_FixedSize}.

These findings indicate that while a significant proportion of repositories align with the GitHub template, many maintainers adapt their policies by tailoring them to the needs of their projects. The inclusion of categories like \texttt{User Guideline} reflects the evolving practices of security policy maintenance, demonstrating an effort to address user-specific concerns and improve overall security.

\begin{tcolorbox}[] \textbf{RQ2 Summary}: Our findings suggest that while a significant portion of developers align with GitHub's security policy guidelines, with 39.93\% of repositories incorporating all three core elements (\texttt{Generic Policy}, \texttt{Reporting Mechanism}, and \texttt{Scope of Practice}), the majority (60.07\%) deviate by omitting one or more of these elements or adding additional categories. This highlights varying levels of adherence and customization among open-source projects, including the notable addition of a \texttt{User Guideline}, which reflects its acknowledged importance. \end{tcolorbox}

% After completing RQ1, where we identified nine distinct categories of security policies, we applied these categories back to the PyPI dataset. For each unique package, we categorized its security policy content blocks based on our predefined categories, resulting in a structured set of categories per package. This structured dataset allowed us to examine patterns and commonalities across repositories.

% To evaluate the significance of these patterns, we focused on the \textit{support} metric. Support measures the frequency of a specific category or combination of categories in the dataset. By analyzing support, we identified the most common and relevant patterns within security policies, providing insights into the foundational components that security policies across repositories often share.

% As shown in Figure~\ref{fig:PyPIARM_FixedSize}, the results of our association rule mining reveal that four categories exhibit strong support and frequently co-occur within security policies: \textit{Generic Policy}, \textit{Reporting Mechanism}, \textit{Scope of Practice}, and \textit{User Guideline}. Interestingly, three of these categories—Generic Policy, Reporting Mechanism, and Scope of Practice—are also found in GitHub's security policy template, which GitHub recommends maintainers use as a foundation for creating their own policies.

% However, the \textit{User Guideline} category, which provides security-related instructions for users, is notably absent from GitHub's template. Despite this, our analysis shows that maintainers frequently include user guidelines alongside the three main categories advised by GitHub. This suggests that maintainers recognize the importance of providing users with specific security guidelines, viewing it as a valuable addition to the standard policy elements. These findings highlight how maintainers go beyond template recommendations to address user needs, enhancing security practices across repositories.

\begin{figure}[h]
    \centering
    \includegraphics[width=.9\linewidth 
    % ,height=0.28\textheight
    ]{PyPIARM_FixedSize2.png}
    \captionsetup{justification=centering}
    \caption{Results from applying association rule mining\\(addressing RQ2)}
    \label{fig:PyPIARM_FixedSize}
\end{figure}

\subsection{RQ3: Does the occurrence of security policy categories correlate with characteristics of software repositories?}

Figure \ref{fig:RQ3Correlations} shows the results of the point-biserial correlation analysis. A positive correlation is observed between repository size and the presence of the \texttt{History of Vulnerability} category, suggesting that larger repositories are more likely to document their vulnerability history. This may be due to the increased complexity and greater likelihood of past security incidents that require tracking and documentation. Similarly, a positive correlation exists between the number of stars and the \texttt{User Guideline} category, indicating that more popular projects, as measured by star count, are more likely to provide specific security instructions for users. Conversely, a negative correlation is seen between the total number of issues and the \texttt{Scope of Practice} category, suggesting that projects with a high volume of issues may place less emphasis on clearly defining the scope of their security coverage.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth
    ,height=0.22\textheight
    ]{RQ3.png}
    \captionsetup{justification=centering}
    \caption{Correlations between project features and the occurrence of security policy categories (addressing RQ3)}
    \label{fig:RQ3Correlations}
\end{figure}

\begin{tcolorbox}[] \textbf{RQ3 Summary}: The analysis reveals correlations between repository characteristics and security policy categories. Larger repositories correlate with the \texttt{History of Vulnerability} category, while popular projects (based on stars) are more likely to include \texttt{User Guideline}. Conversely, repositories with many issues tend to emphasize the \texttt{Scope of Practice} category less. \end{tcolorbox}

% 
% After categorizing security policies into nine distinct categories in RQ1, we applied point-biserial correlation analysis to understand how these security policy categories correlate with various repository characteristics as shown in figure \ref{fig:RQ3Correlations}.

% Our analysis reveals notable correlations between repository characteristics and specific elements within security policies, particularly focusing on popularity and scope of practice.

% Repositories with a high number of stars, reflecting significant community attention and user interest, tend to include a \textit{User Guideline} section in their security policies. This guideline provides essential instructions and best practices, which help users understand secure usage and contribute responsibly to the project. The presence of user guidelines in highly-starred repositories suggests that maintainers recognize the importance of offering clear, accessible security information to a broad user base. This addition is likely an effort to ensure that a diverse audience, drawn to the project by its popularity, adheres to secure practices.

% Furthermore, our analysis indicates that repositories lacking a \textit{Scope of Practice} in their security policies tend to experience more open issues. Without a defined scope, users may not know which versions are actively maintained, leading to confusion and potentially unnecessary issue reports. By not specifying which parts of the project are covered under security maintenance, maintainers may inadvertently invite a higher volume of issues from users unsure about the project’s support boundaries. This suggests that a well-defined scope of practice can help manage user expectations and streamline issue reporting, ultimately reducing maintenance overhead.

% In addition to these observations, our analysis shows a significant correlation between project size and the inclusion of a \textit{History of Vulnerability} section in security policies. Larger projects, with extensive codebases and complex dependencies, are more likely to experience and document vulnerabilities over time. This documentation provides a clear record of past security issues and their resolutions, helping maintainers and contributors monitor the security landscape of the project. Including a history of vulnerabilities supports transparency and accountability, which can be particularly valuable for large projects where users and developers benefit from a documented security history.

% These findings highlight how maintainers adapt their security policies based on repository characteristics. Popular repositories often include user guidelines to meet the needs of a large audience, ensuring users have access to essential security practices. Projects with well-defined scopes of practice help clarify support boundaries, reducing confusion and unnecessary issue reports from users. Additionally, larger projects are more likely to document a history of vulnerabilities, providing a transparent record of past security issues and resolutions. This approach supports both community engagement and efficient project management, aligning security policies with the unique demands of each repository.



==> sections/5_conclusion.tex <==
\section{Challenges, Opportunities and Future Work}

Our research reveals that many open-source projects require more information when addressing security-related issues, sparking a broader conversation about best practices in security management, especially for OSS projects.
This study investigates the security policies of open-source projects, exploring their characteristics and relationships to project attributes. 

We believe that this work represents a crucial first step in understanding the requirements for effective security measures, their impact on project outcomes, and which policies are actually followed. Additionally, we aim to explore how software communities, such as library ecosystems like NPM, PyPI and so on, conform to these policies.
Future studies will build upon this research by conducting an in-depth analysis of the relationship between security issue resolution and discussions with developers. Furthermore, a larger-scale study of software projects at the ecosystem level will provide valuable insights into how open-source communities navigate and adhere to security policies.



% \pooh{For future work,\\ 
% -the low-hanging fruit one is going to be exploring other ecosystems.\\
% -Investigate the characteristics of security policy from GitHub alternative (other git hosting service. Im not sure the population would be sufficient).\\
% -Tracking for the adoption of practices after this paper was published? maybe this one is too far fetch.
% }


% This research offers a focused analysis of security policies in open-source projects on GitHub, exploring both the structure and content of these documents. By categorizing policy elements and examining their associations, we identified common patterns and key areas frequently addressed in these policies. Our findings highlight that, while the inclusion of security policies is on the rise, the content often varies in depth and scope, suggesting that more standardized guidelines could benefit project maintainers by providing clear expectations for essential security topics.

% Through a structured categorization process involving multiple researchers, we achieved a high level of reliability, ensuring that our results accurately reflect common practices across diverse projects. This process, validated with inter-rater reliability measures, strengthens our conclusions and provides a reliable framework that future researchers can build on. Additionally, our use of association rule mining revealed valuable insights into frequently linked policy elements, offering a clearer view of how security practices are organized within open-source documentation.

% Overall, this study underscores the need for clear and comprehensive security policies in open-source projects. Our findings provide practical recommendations for developers and maintainers, helping them prioritize essential security elements and improve policy consistency. Future research could extend this work by exploring security policies in different ecosystems, examining how various platforms, programming languages, and community norms influence security practices. This broader perspective could further support the open-source community in developing adaptable and effective security standards across ecosystems.


% \textbf{Future Work}

% \section*{Acknowledgment}
% The preferred spelling of the word ``acknowledgment'' in America is without % an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. % G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor % acknowledgments in the unnumbered footnote on the first page.




==> sections/Tables_VersionControl.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{lp{4.75cm}}
\toprule
\textbf{Category} & \textbf{Definition} \\
\midrule
\textbf{Generic policy} & Outline objective and foundation of security policy. \\
\textbf{Reporting mechanism} & A set of instructions outlining the procedure for reporting security vulnerabilities to the relevant developers. \\
\textbf{Information on maintainer} & Maintainer information e.g. name, email, role, responsibility. \\
\textbf{Scope of practice} & The list of project versions still under maintenance. \\
\textbf{Project practice} & Detailed procedural steps that will be executed when a vulnerability is reported. \\
\textbf{History of vulnerability} & A list of disclosed vulnerabilities. \\
\textbf{User guideline} & Security related and project specific e.g. Instructions for users, including secure usage of dependencies, recommended configurations, and general project usage. \\
\textbf{Additional information} & Non-security related and project specific e.g. Access for further details that are non-related to the security, Copyright section, project contribution, acknowledgement. \\
\textbf{Others} & None of all above. \\
\bottomrule
\end{tabular}
\caption{Categories of Security Policy Titles}
\label{}
\end{table}

\begin{table*}[!]
\centering
\begin{tabular}{lrl}
\toprule
\textbf{Category} & \textbf{Count} & \textbf{Example} \\
\midrule
\textbf{Reporting mechanism} & 282 & \makecell[l]{"To report a vulnerability, please do not share it publicly on GitHub
nor the community slack channel.\\ Instead, contact the \censortext \ \ team
directly via email first: \censortext"} \\\\
\textbf{Generic policy} & 211 & \makecell[l]{"This document describes model security and code security in \censortext.\\ It also provides guidelines on how to report vulnerabilities in \censortext."} \\\\
\textbf{User guideline} & 133 & \makecell[l]{"\censortext \ \ is not intended to be deployed on a public-facing server.\\ By default the web UI is only exposed on localhost, so normally this is not a problem.\\
Do not give someone access to the web UI unless you trust them with everything else that is on that machine."} \\\\
\textbf{Scope of practice} & 127 & \makecell[l]{"These \censortext \ \ releases are currently supported with security updates:\\
Version 2.0.x - \texttimes\  (not released)\\
Version 1.2.x - \checkmark\  Supported\\
Version 1.1.x - \texttimes\  Not supported\\
Version \textless{}1.1 - \texttimes\ Not supported"} \\\\
\textbf{Project practice} & 20 & \makecell[l]{"Each report is acknowledged and analyzed by security response members within five (5) working days.\\
Any vulnerability information shared with security response members stays within the \censortext \ \ project and-\\ will not be disseminated to other projects unless it is necessary to get the issue fixed.\\
As the security issue moves from triage, to identified fix, to release planning we will keep the reporter updated."} \\\\
\textbf{History of vulnerability} & 8 & \makecell[l]{"We maintain Security Advisories on the \censortext \ \ project \censortext \ \  repository,\\
where we will post a summary, remediation, and mitigation details\\ for any patch containing security fixes."} \\\\
\textbf{Additional information} & 7 & "We prefer all communications to be in English." \\\\
\textbf{Information on maintainer} & 4 & \makecell[l]{"\censortext \ \ is always open to feedback, questions, and suggestions.\\ If you would like to talk to us, please feel free to email us at \censortext \ \,\\ and our PGP key is at \censortext \ ."} \\\\
\textbf{Others} & 0 & -- \\
\midrule
\textbf{Total} & 722 &  \\
\bottomrule
\end{tabular}


\caption{Distribution of Security Policy Categories in PyPI Population}
\label{}
\end{table*}


\begin{table*}[!]
\centering
\begin{tabular}{lll}
\toprule
\textbf{Category} & \textbf{Definition} & \textbf{Example} \\
\midrule
\textbf{Reporting mechanism} & \makecell[tl]{A set of instructions outlining\\ the procedure for reporting\\ security vulnerabilities to the\\ relevant developers.} & \makecell[tl]{``To report a vulnerability, please do not share it publicly on GitHub nor\\ the community slack channel. Instead, contact the \censortext \\ team directly \\via email first: \censortext \ ''} \\

\textbf{Generic policy} & \makecell[tl]{Outline objective and foundation \\of security policy.} & \makecell[tl]{``This document describes model security and code security in \censortext.\\ It also provides guidelines on how to report vulnerabilities in \censortext.''} \\

\textbf{User guideline} & \makecell[tl]{Security-related and project-\\specific e.g. Instructions for\\ users, including secure usage\\ of dependencies, recommended\\ configurations, and general\\ project usage.} & \makecell[tl]{``\censortext \ \ is not intended to be deployed on a public-facing server.\\ By default the web UI is only exposed on localhost, so normally this is \\not a problem. Do not give someone access to the web UI unless you\\ trust them with everything else that is on that machine.''} \\

\textbf{Scope of practice} & \makecell[tl]{The list of project versions still\\ under maintenance.} & \makecell[tl]{``These \censortext \ \ releases are currently supported with security updates:\\ Version 1.2.x - \checkmark\  Supported\\ Version \textless{}1.1 - \texttimes\ Not supported''} \\

\textbf{Project practice} & \makecell[tl]{Detailed procedural steps that will\\ be executed when a vulnerability \\is reported.} & \makecell[tl]{``Each report is acknowledged and analyzed by security response members\\ within five (5) working days. Any vulnerability information shared with\\ security response members stays within the \censortext \ \ project and will not be\\ disseminated to other projects unless it is necessary to get the issue fixed.''} \\

\textbf{History of vulnerability} & \makecell[tl]{A list of disclosed vulnerabilities.} & \makecell[tl]{``We maintain Security Advisories on the \censortext \ \ project \censortext \ \ repository,\\ where we will post a summary, remediation, and mitigation details\\ for any patch containing security fixes."} \\

\textbf{Additional information} & \makecell[tl]{Non-security related and project\\ specific e.g. Access for further\\ details that are non-related to the\\ security, Copyright section, project\\ contribution, acknowledgment.} & \makecell[tl]{``We prefer all communications to be in English''} \\

\textbf{Information on maintainer} & \makecell[tl]{Maintainer information e.g. name, \\email, role, responsibility.} & \makecell[tl]{``\censortext \ \ is always open to feedback, questions, and suggestions.\\ If you would like to talk to us, please feel free to email us at \censortext \ \,\\ and our PGP key is at \censortext \ .''} \\

\textbf{Others} & \makecell[tl]{None of all above.} & - \\

\bottomrule
\end{tabular}
\caption{Categories of Security Policy Titles}
\label{}
\end{table*}
